Multi-Channel Operation for the Release 2 of ETSI Cooperative Intelligent Transport Systems

Vehicles and road infrastructure are starting to be equipped with vehicle-to-everything (V2X) communication solutions to increase road safety and provide new services to drivers and passengers. In Europe, the deployment is based on a set of Release 1 standards developed by ETSI to support basic use cases for cooperative intelligent transport systems (C-ITS). For them, the capacity of a single 10 MHz channel in the ITS band at 5.9 GHz is considered sufficient. At the same time, the ITS stakeholders are working towards several advanced use cases, which imply a significant increment of data traffic and the need for multiple channels. To address this issue, ETSI has recently standardized a new multi-channel operation (MCO) concept for flexible, efficient, and future-proof use of multiple channels. This new concept is defined in a set of new specifications that represent the foundation for the future releases of C-ITS standards. The present paper provides a comprehensive review of the new set of specifications, describing the main entities extending the C-ITS architecture at the different layers of the protocol stack, In addition, the paper provides representative examples that describe how these MCO standards will be used in the future and discusses some of the main open issues arising. The review and analysis of this paper facilitate the understanding and motivation of the new set of Release 2 ETSI specifications for MCO and the identification of new research opportunities.

==> Sections/2_MCO_Preliminaries_backup.tex <==
\section{MCO Preliminaries}\label{sec:preliminaries}

\subsection{Channels and interference} 

In most countries worldwide, spectrum has been allocated specifically for direct \ac{V2X} communications. With few exceptions, it mainly consists of a group of 10~MHz channels around 5.9~GHz, also known as \ac{ITS} band. 
%The use of pairs of them to obtain 20~MHz wide channels is an option currently under debate. 
Spectrum at higher frequency (e.g., around 60~GHz in Europe) is being allocated for the so-called mmWave communication. 

Focusing on the ITS band at 5.9~GHz in Europe, which is the target of the MCO specifications, the latest regulations\footnote {Implementing Decision 2020/1426 of the European Commission, October 2020.} 
reserve for road applications seven 10~MHz channels between 5.855~GHz and 5.925~GHz, named \acp{SCH}. These channels are summarized in Fig.~\ref{fig:channels}. Among them, the one between 5.895 and 5.905~GHz (SCH0) is the one primarily used by the Release~1 safety applications (including \acp{CAM} and \acp{DENM}), which was originally referred to as \ac{CCH}. The two lowest channels (SCH3 and SCH4) are assigned as non-safety channels. Finally, the highest one (SCH6) is subject to priority to urban rail systems, and can therefore be used by vehicles only under specific conditions. The 10~MHz just above this designated spectrum (i.e. between 5.925~GHz and 5.935~GHz) is also allocated to ITS, but assigned to urban rail.

\begin{figure*}[t]
\centering
\includegraphics[scale=0.6, draft=false]{Figures/channels_v3}
\caption{Allocation of the channels in the ITS band around 5.9 GHz in Europe.}
\label{fig:channels}
\end{figure*}

Given the non-ideality of communication equipment, the transmissions performed in one channel cause unwanted emissions on nearby channels, which impact differently depending on the channel separation. 
It has been shown, e.g. in~\cite{Campolo_ACI}, that the interference is negligible when channels are separated by a gap of 10~MHz or more. In contrast, communication reliability reduces when the channels are adjacent. It is shown in ETSI~TR~103~439, through simulations assuming ITS-G5 in a highway scenario, that the maximum distance between source and destination to have 90\% packet reception probability reduces by up to 40\% when two adjacent channels are highly loaded. 

\bazziremove{The conclusions from the studies on interference 
suggest preferring non-adjacent channels for simultaneous transmissions if possible; for example, the use of SCH0 is preferable with SCH1 instead of SCH2 (see Fig.~\ref{fig:channels}). It is also observed in ETSI TR 103 439 that more stringent limitations to the load in one channel can provide a benefit in terms of reduced average interference to the adjacent ones. In contrast,  different constraints on the transmission power may have a low impact.}

\subsection{Access Technologies}

\bazziremove{The ITS spectrum is reserved for direct \ac{V2X} communications among nearby road entities. The reservation is related to the usage but agnostic to radio technologies.}

\bazzi{The reservation of the ITS spectrum for direct \ac{V2X} communications is related to the usage but agnostic to radio technologies.} Currently, two main families of standards are available and subject to hard debates. The first family is based on the IEEE~802.11p amendment. 
Defined in 2010 and now part of IEEE~802.11-2020, it is a fully distributed and asynchronous technology relying on \ac{CSMA/CA} at the \ac{MAC}. \bazziremove{Several studies and large-scale experiments have proven reliability for the ``Day-1'' use cases with a spatial range of several hundreds of meters in \ac{LOS} conditions cite{Boban_VNC2014}.} In Europe, IEEE~802.11p is part of the ITS-G5 access technology (ETSI EN~302~663). %that is already deployed on some car models.
In 2018, IEEE formed a new working group to specify a new amendment, called IEEE~802.11bd, expected to be published by early 2023. IEEE~802.11bd enhances reliability and range, while maintaining backward compatibility~\cite{8723326}.

The second family belongs to the cellular ecosystem and consists of two different standards, i.e., LTE-V2X sidelink as part of the 4$^\text{th}$ generation and NR-V2X sidelink as part of the 5$^\text{th}$ generation (ETSI~TR~137~985). These two access technologies share very similar principles, with some features added in NR-V2X to better manage aperiodic traffic and large packets \cite{GarMolBobGozColSahKou:21}. Both technologies make use of multi-carrier-based multiple access %\ac{OFDMA} 
and therefore require timely synchronization, primarily based on \acp{GNSS}. 
The radio resource allocation can be either autonomously determined by the devices or controlled by the network, with the former case normally considered for the ITS band.
%, each device is expected to look at the recent past to estimate which resources will be available in the near future with the lowest interference.
\hl{One sentence about C-V2X roadmap to be added.}
\jonas{On the C-V2X roadmap, the next steps are the integration of pedestrians and enhanced QoS }

To date, in Europe, no restrictions have been defined for the use of the channels by either technology. Work has been done to investigate the co-channel coexistence, leading to proposals for modifications to mitigate the mutual interference (ETSI TR~103~667 and ETSI TR~103~766); however, an agreement has not yet been reached on any of them. 

\subsection{Background on MCO}

\hl{AB: in my opinion, the description of 1609.4 can be reduced if we need room.}

\hl{Possible new references to be added:} \cite{9079451} \cite{7875465} \cite{s19153283} 
%Ref. \cite{kwon2016improving} with RSUs that coordinate the use of the SCHs
%Ref. \cite{9621146} not considered - it is a conference paper with very limited details
%Ref. \cite{9311814}  is more multi-RAT than multi-channel

MCO is not a new concept. IEEE specified an MCO scheme in IEEE~1609.4
as part of the \ac{WAVE} standards \cite{Kenney_DSRCstandards}.
WAVE includes channel coordination, channel routing,
and QoS parameter mapping 
using the enhanced distributed channel access (EDCA) in the data plane. The management plane specifies several MCO-related services, among which: \emph{(i)} multi-channel synchronization of WAVE devices via Time Advertisement frames, \emph{(ii)} channel access control, and \emph{(iii)} changing of the MAC address to support pseudonymity. IEEE~1609.4 relies on two types of channels, i.e. the \ac{CCH} and the \acp{SCH}. The CCH may be used by the \ac{WSMP} only. SCHs may be used by \ac{WSMP} and/or IPv6. %IEEE 1609.4 does not specify if a device has to be on a specific time at a specific channel: a device can stay on one channel all the time or can change to any other channel in the next time slot. 
In contrast to the MCO framework in this paper, IEEE~1609.4 is specific to a single access technology and tightly linked to the WAVE standards.

Besides standardization, MCO has been considered in research. In~\cite{Haerri2015} and \cite{Campolo_MCO_servey}, the authors provide an overview of the MCO-related standardization activities at that time in Europe and the US. 
They also describe the channel allocation and switching principles, including synchronous and asynchronous approaches, based on distributed channel management and \acp{SAM}. \jonas{In \cite{9079451}, based on \ac{WAVE} a two-transceiver approach is introduced with the distribution of available resources information on the SCHO for all other service channels. The authors in \cite{7875465} define flexible scheduling of safety and non-safety messages on both the SCO and the other service channels coordinated by an RSU based on a single transceiver and \ac{WAVE}. \cite{s19153283}  defines a new MAC to select a non-shard or a shard channel for each vehicle transmission. It emphasizes the throughput but does not consider the coordination for the reception. All three proposals do not take into account the application requirements and different access technologies.} The authors of \cite{BOBAN201617} present an approach for service-actuated multi-channel operation for vehicular communications (SAMCO) with asynchronous channel switching. 
They use \acp{SAM} to distribute service information, whereas a station can prioritize the selection of services based on user preferences and channel load. SAMCO assumes that all systems are equipped with dual transceivers, with one transceiver continuously listening to the CCH, and assumes that services are in pre-defined categories. The authors in~\cite{Sepulcre_CarHet} describe a technology and application-agnostic, distributed, context-aware heterogeneous \ac{V2X} communication system (CARHet).
The proposed channel selection algorithm allows every station to dynamically choose the appropriate access technology and channel based on the application requirements. 
CARHet assumes that all vehicles can transmit and listen to all channels (i.e. they have as many radio interfaces as channels) and focuses on balancing the load among the different channels to minimize interference and packet losses. All these existing MCO schemes have been considered and taken into account for developing our proposed MCO framework.



==> Sections/6_Open_issues_backup-version.tex <==
\section{Open Issues}
\label{sec:openissues}

The designed MCO concept is a core concept of the C-ITS protocol stack for Release~2 and therefore brings modifications to all layers of the C-ITS protocol stack. Thereby, new issues and challenges in research, standardization, and deployment arise, from which we highlight three aspects. 

\textbf{MCO congestion control}: Because of the safety-related requirements, mechanisms to manage channel congestion should be mainly at the functional level, i.e., in the facilities layer. In Release~1, congestion control is instead only realised by discarding messages at the access layer \cite{Smely2015}.
With more channels, multiple access technologies, and various additional applications, the access layer does not have the required comprehensive information. For Release~2, it is envisioned that the access layer should be used as a strict enforcer of the legislation to access the channel, i.e. the Radio Equipment Directive (RED) and the harmonized ETSI EN~302~663. More intelligent resource management must be realized at the facilities layer with the BME sharing resources among the applications efficiently and controlling their message generation. 

\textbf{Channel association}: 
The assignment of services to the available channels in the 5.9~GHz frequency band requires coordination across all C-ITS stations. In a simple scheme, services have predefined channel associations with the corresponding facilities layer service. This scheme does not exist yet and should be realized as a collaboration between all stakeholders as part of the standards. Future evolution of the MCO concept could include more dynamic and advanced solutions that dynamically adapt to the vehicular context. A solution that is able to balance the load among the available channels can be considered the optimum one because it minimizes interference and packet collisions. However, the number of channels that can be simultaneously used depends on the number of radio interfaces implemented. If all C-ITS stations implement the same number of radio interfaces, solutions such as \cite{Sepulcre_CarHet} could be applied. However, in practical scenarios, differently configured C-ITS stations are expected to coexist, and this represents a significant challenge that requires further investigation.

\textbf{Exchange of perceived channel state}: In Release 1, ITS-G5 already enables the exchange of the locally perceived channel status with other stations. However, this option was practically not deployed. For Release~2, it is expected that this  state exchange will become more relevant. For example, even if a transceiver of a station is not tuned to a channel, other stations could provide information regarding the state of this channel. This information could then be used to predict future channel conditions and realize better decisions on which channel to tune its transceivers. %, with the aim to grant the necessary quality of service to the applications.

%Andreas: I suggest moving a shorter version of this to the conclusions
%\festagremove{\textbf{Standardization}: The Release 2 set of specifications for the C-ITS protocol stack is under active development. The MCO set of standards realized are in an advance state in comparison to other Release~2 draft  standards. Some terms and the general architecture of the protocol stack may face significant changes in comparison to Release~1, e.g., channel naming where the Control CHannel (CCH) is reamed to SCH0. Some of the under development Release 2 standards will have an influence on the MCO standards. For example, it is expected that security will have to be better integrated across the MCO standards. A lot of work will be required to align the MCO standards with the future finished Release 2 set of specifications.} 

%\festagremove{Furthermore, these issues and new research opportunities open the way to research using other type of framework, such as Artificial Intelligence.}

\begin{comment}
Also, in an outlook it could be discussed that the MCO concept impacts other functions, such as DCC which will need to be changed in the future.

Research opportunities.

\bazzi{AB notes: congestion control is normally a feature at the higher layers in IP networks, but mostly treated at the lower layers in V2X. With the presence of multiple channels and possibly multiple technologies, it necessarily becomes an issue to be managed at the facilities layer. Whereas some work has been done in this direction...}

\delooz{Discuss that the Facilities layer is the key layer, MCO does not bring major change currently at the lower layer}
\delooz{QD: discuss how to use the available data from lower layers (e.g., location table at the N\&T layer)}
\delooz{QD: Emphasize that AI could be used, e.g., evaluate or distribute resources among the services:)}
\delooz{QD: discuss the potential of load balancing using additional mechanism such as SA}

\end{comment}

